Self-Supervised Scene Dynamic Recovery from Rolling Shutter Images and Events

Scene Dynamic Recovery (SDR) by inverting distorted Rolling Shutter (RS) images to an undistorted high frame-rate Global Shutter (GS) video is a severely ill-posed problem due to the missing temporal dynamic information in both RS intra-frame scanlines and inter-frame exposures, particularly when prior knowledge about camera/object motions is unavailable. Commonly used artificial assumptions on scenes/motions and data-specific characteristics are prone to producing sub-optimal solutions in real-world scenarios. To address this challenge, we propose an event-based SDR network within a self-supervised learning paradigm, i.e., SelfUnroll. We leverage the extremely high temporal resolution of event cameras to provide accurate inter/intra-frame dynamic information. Specifically, an Event-based Inter/intra-frame Compensator (E-IC) is proposed to predict the per-pixel dynamic between arbitrary time intervals, including the temporal transition and spatial translation. Exploring connections in terms of RS-RS, RS-GS, and GS-RS, we explicitly formulate mutual constraints with the proposed E-IC, resulting in supervisions without ground-truth GS images. Extensive evaluations over synthetic and real datasets demonstrate that the proposed method achieves state-of-the-art and shows remarkable performance for event-based RS2GS inversion in real-world scenarios. The dataset and code are available at https://w3un.github.io/selfunroll/.

==> Figs/Gev-RS-inter-intra-sequence.tex <==

\def\imwidth{0.187}
\def\cimwid{0.13}
\def\rswidth{0.23}
\def\zuoxia{(-1.5,-1.15)}
\def\youshang{(-0.6,-0.45)}
\def\seqwidth{0.35}
\def\ssyy{(-0.8,-0.85)}
\def\ssizz{0.5cm}
\def\sswidth{0.245\textwidth}
\def\ssmag{3}
\def\scc{(2.12,1.4)}
\def\boxseq{0.44}
\def\boxseqq{0.48}
%  \def\areaddd{{0 0 0 0}}
\begin{figure*}[!t]
\footnotesize
	\centering

    % \subfigure{
%     	\begin{minipage}[t]{\imwidth\linewidth}
%     		\centering
%     		\begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
% 				\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/rssr/rssr_intra1_2.png}};
% 				% \spy on \ssxxs in node [left] at \ssyys;
% 				\draw[green] \zuoxia rectangle \youshang;
% 				\end{tikzpicture}
			
% 			(a) RSSR\vspace{0.5em}
%     	\end{minipage}%
%     \hfill
%     	\begin{minipage}[t]{\imwidth\linewidth}
%     		\centering
%     	    \begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
% 				\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/cvr/cvr_intra1_2.png}};
% 				% \spy on \ssxxs in node [left] at \ssyys;
% 				\draw[green] \zuoxia rectangle \youshang;
% 				\end{tikzpicture}
% 			(b) CVR\vspace{0.5em}
%     	\end{minipage}%
%     \hfill
%     	\begin{minipage}[t]{\imwidth\linewidth}
%     		\centering
%     	    \begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
% 				\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/timelens/intra1_2.png}};
% 				% \spy on \ssxxs in node [left] at \ssyys;
% 				\draw[green] \zuoxia rectangle \youshang;
% 				\end{tikzpicture}
% 			(c) EvUnroll\vspace{0.5em}
%     	\end{minipage}%
%     \hfill
% 		\begin{minipage}[t]{\imwidth\linewidth}
% 			\centering
% 			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
% 				\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/selfunroll/intra1_S2.png}};
% 				% \spy on \ssxxs in node [left] at \ssyys;
% 				\draw[green] \zuoxia rectangle \youshang;
% 				\end{tikzpicture}
% 			(d) SelfUnroll-S\vspace{.5em}
			
% % 			(27.60/26.49, 0.8318/0.7907)\\
			
% 		\end{minipage}%
% \hfill
% \begin{minipage}[t]{\imwidth\linewidth}
%     		\centering
%     		\begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
% 				\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/selfunroll/intra1_M2.png}};
% 				% \spy on \ssxxs in node [left] at \ssyys;
% 				\draw[green] \zuoxia rectangle \youshang;
% 				\end{tikzpicture}
			
% 			(e) SelfUnroll-M\vspace{0.5em}
%     	\end{minipage}%
%  \hfill
% \vspace{6em}
  \begin{minipage}[t][3.3cm]{\rswidth\textwidth}
  \vspace{0pt}
    		\centering
      % \vspace{0.4em}
    		%ground truth
              
            % \vspace{0.8em}
    		%ground truth
              
   %          % \vspace{0.8em}
   %                  % RS frame \vspace{-0.3em}
             
             % \begin{table}[T]{0.8\linewidth}
%  \renewcommand\arraystretch{2}
% \\
%  \begin{tabular}{l|l}
% \multicolumn{1}{c|}{\makecell[c]{(a) Overlap of \\RS frames}} & (b) CVR                  \\ \cline{2-2} 
%                         & \multirow{2}{*}{\makecell[l]{(c) EvUnroll\\+Timelens}} \\
%                         &                    \\ \cline{2-2} 
%                         & (d) SelfUnroll-M                 \\ \cline{2-2} 
%                         & (e) Ground Truth                 
% \end{tabular}
% \begin{tabular}{c|l}
% \multirow{4}{*}{\makecell[c]{(a) Overlap of \\RS frames}} & (b) CVR \\ \cline{2-2} 
%                     & \makecell[l]{(c) EvUnroll\\+Timelens}\\ \cline{2-2} 
%                     & (d) SelfUnroll-M\\ \cline{2-2} 
%                     & (e) Ground Truth
% \end{tabular}
% \end{table}
% \vspace{3em}
\begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
\tikzstyle{every node}=[font=\footnotesize]
        				\node [label= {[label distance=0.1cm,text depth=2.3ex,align=center] below:\textcolor{black}{ {Input frame $I_{1}^{RS}$}}}]{\includegraphics[width=\linewidth,trim={10 0 80 0},clip]{Figs/img/inter-intra-seq/selfunroll/rs1.png}};
        				% \spy on \ssxxs in node [left] at \ssyys;
        				\draw[green] \zuoxia rectangle \youshang;
        				\end{tikzpicture}


            
            \begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
\tikzstyle{every node}=[font=\footnotesize]
        				\node [label= {[label distance=0.1cm,text depth=2.3ex,align=center] below:\textcolor{black}{ {Input frame $I_{2}^{RS}$}}}]{\includegraphics[width=\linewidth,trim={10 0 80 0},clip]{Figs/img/inter-intra-seq/selfunroll/rs2.png}};
        				% \spy on \ssxxs in node [left] at \ssyys;
        				\draw[green] \zuoxia rectangle \youshang;
        				\end{tikzpicture}
% \begin{tabular}{l|l}
% \hline
%  (a) CVR\cite{fan2022context}&(b) EvUnroll\cite{zhou2022evunroll}+\cite{tulyakov2021time} \\ \hline
%  (c) SelfUnroll-M& (d) GT  \\ \hline
% \end{tabular}
%  \begin{tabular}{l|l}
% (a) previous frame $I^{RS}_1$  & {\makecell[l]{(d) EvUnroll\cite{zhou2022evunroll}\\+Timelens\cite{tulyakov2021time}}} \\ \hline
%                   % &                   \\ \cline{2-2} 
%             (b) next frame $I^{RS}_2$       &     (e) SelfUnroll-M               \\ \hline
%        (c) CVR\cite{fan2022context}           &       (f) Ground Truth            
% \end{tabular}
            % (a) \vspace{0.3em}
			% \begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
			% 	\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/selfunroll/rs2.png}};
			% 	% \spy on \ssxxs in node [left] at \ssyys;
			% 	% \draw[green] \zuoxia rectangle \youshang;
			% 	\end{tikzpicture}
            
   %         RS2 frame\vspace{0.3em}
   %         \begin{tikzpicture}[spy using outlines={rectangle,green,magnification=\ssmag,size=\ssizz},inner sep=0]
   %      				\node {\includegraphics[width=\linewidth]{Figs/img/inter-intra-seq/selfunroll/intra1_GT2.png}};
   %      				% \spy on \ssxxs in node [left] at \ssyys;
   %      				% \draw[green] \zuoxia rectangle \youshang;
   %      				\end{tikzpicture}
            
   %          GT\vspace{0.3em}
    	\end{minipage}% 
     % \hill
\hspace*{0em}
% \begin{minipage}
%     \begin{table}[]
%         \centering
%         \begin{tabular}{c|c}
%              &  \\
%              & 
%         \end{tabular}
%         \caption{Caption}
%         \label{tab:my_label}
%     \end{table}
% \end{minipage}
\begin{minipage}[t]{0.255\textwidth}
            \vspace{0pt}
    		\centering
      % trim={左，下，右，上}
      % \begin{tikzpicture}[inner sep=0]
      %       \node [label={[label distance=0.25cm,text depth=-1ex,rotate=90]right: \textcolor{black}{\scriptsize {(a)}}}] at (0,8.7) {};
      %       \end{tikzpicture}
			% \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_intra1_1.png}
   %      \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_intra1_2.png}\\
   \begin{tikzpicture}[inner sep=0]
   \tikzstyle{every node}=[font=\scriptsize]
            \node[
            label= {[label distance=-0.3cm,text depth=2.3ex,align=center,rotate =90] left:\textcolor{black}{ {CVR}}}]{\includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_intra1_1.png}};
            \end{tikzpicture}
   \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_intra1_2.png}\\\vspace{.5mm}
            % \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/intra1_1.png}
            % \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/intra1_2.png}\\
            \begin{tikzpicture}[inner sep=0]
   \tikzstyle{every node}=[font=\scriptsize]
            \node[
            label= {[label distance=-0.5cm,text width=1cm,text depth=2.3ex,align=center,rotate = 90] left:\textcolor{black}{ {EvUnroll }}}]{\includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/intra1_1.png}};
            \end{tikzpicture}
            \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/intra1_2.png}\\\vspace{.5mm}
            \begin{tikzpicture}[inner sep=0]
            \tikzstyle{every node}=[font=\scriptsize]
            \node[
            label= {[label distance=-0.7cm,text depth=2.3ex,align=center,rotate = 90] left:\textcolor{black}{ {SelfUnroll-M}}}]{\includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra1_M1.png}};
            \end{tikzpicture}
            \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra1_M2.png}\\\vspace{.5mm}
            \begin{tikzpicture}[inner sep=0]
            \tikzstyle{every node}=[font=\scriptsize]
            \node[
            label= {[label distance=-0.3cm,text depth=2.3ex,align=center,rotate = 90] left:\textcolor{black}{ {GT}}}]{\includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra1_GT1.png}};
            \end{tikzpicture}
            \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra1_GT2.png}\\\vspace{.5mm}
             Intra-frame of $I^{RS}_{1}$
\end{minipage}
\hspace{0.01em}
\vrule % 竖直分割线
\hspace{0.01em}
\begin{minipage}[t]{0.235\textwidth}
            \vspace{0pt}
    		\centering
      % trim={左，下，右，上}
      % \begin{tikzpicture}[inner sep=0]
      %       \node [label={[label distance=0.25cm,text depth=-1ex,rotate=90]right: \textcolor{black}{\scriptsize {(a)}}}] at (0,8.7) {};
      %       \end{tikzpicture}
			% \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_inter0.png}
   % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_inter1.png}
        % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_inter2.png}\\
			\includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_inter0.png}
   % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_inter1.png}
   \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_inter2.png}\\\vspace{.5mm}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/0064.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/0065.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/0066.png}\\
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/000064.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/000065.png}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/000066.png}\\\vspace{.5mm}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_S0.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_S1.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_S2.png}\\
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_M0.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_M1.png}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_M2.png}\\\vspace{.5mm}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_GT0.png}
            % \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_GT1.png}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/inter_GT2.png}\\\vspace{.5mm}
            Inter-frame of $I^{RS}_{1}$ and $I^{RS}_{2}$
\end{minipage}
\hspace{0.01em}
\vrule % 竖直分割线
\hspace{0.01em}
\begin{minipage}[t]{0.235\textwidth}
            \vspace{0pt}
    		\centering
      % trim={左，下，右，上}
      % \begin{tikzpicture}[inner sep=0]
      %       \node [label={[label distance=0.25cm,text depth=-1ex,rotate=90]right: \textcolor{black}{\scriptsize {(a)}}}] at (0,8.7) {};
      %       \end{tikzpicture}
			% \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_intra2_1.png}
   %      \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/rssr/rssr_intra2_2.png}\\
			\includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_intra2_1.png}
   \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/cvr/cvr_intra2_2.png}
   \\\vspace{.5mm}
            % \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/intra2_1.png}
            % \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/dain/intra2_2.png}\\
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/intra2_1.png}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/timelens/intra2_2.png}
            \\\vspace{.5mm}
            % \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra2_S1.png}
            % \includegraphics[width=\boxseq\linewidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra2_S2.png}\\
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra2_M1.png}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra2_M2.png}
            \\\vspace{.5mm}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra2_GT1.png}
            \includegraphics[width=\boxseqq\textwidth,trim={100 35 360 180},clip]{Figs/img/inter-intra-seq/selfunroll/intra2_GT2.png}\\\vspace{.5mm}
              Intra-frame of $I^{RS}_{2}$
\end{minipage}
% }

	\caption{Qualitative comparisons of intra-/inter-frame GS video sequence restorations on the {Gev-RS} dataset. }
	\label{mul_image}
\end{figure*}


==> Tables/MOA.tex <==
\begin{table}[!htb]
\caption{Ablation study of multi-frame fusion strategy on the {Gev-RS} dataset. SelfUnroll-S can reconstruct the GS images from each of two consecutive RS frames and the $\times$ represents the better reconstruction. \textcolor{red}{\textbf{Bold}} numbers represents the best performance.}
\centering
\resizebox{0.68\linewidth}{!}{
\begin{tabular}{cccc}

\hline
Fusion & PSNR$\uparrow$     & SSIM$\uparrow$    & LPIPS$\downarrow$   \\ \hline
     $\times$    & 32.26 & 0.926 & 0.0204 \\ 
    Average    & 32.26 & 0.928 & 0.0305 \\
    MOA   & \textcolor{red}{\textbf{32.62}}  & \textcolor{red}{\textbf{ 0.932 }} & \textcolor{red}{\textbf{0.0200 }} \\ \hline
\end{tabular}
}
\vspace{-1em}

\label{ablation_MOA}
\end{table}
